Bayesian Paired-Comparison with the bpcs Package

This article introduces the bpcs R package (Bayesian Paired Comparison in Stan) and the statistical models implemented in the package. This package aims to facilitate the use of Bayesian models for paired comparison data in behavioral research. Bayesian analysis of paired comparison data allows parameter estimation even in conditions where the maximum likelihood does not exist, allows easy extension of paired comparison models, provide straightforward interpretation of the results with credible intervals, have better control of type I error, have more robust evidence towards the null hypothesis, allows propagation of uncertainties, includes prior information, and perform well when handling models with many parameters and latent variables. The bpcs package provides a consistent interface for R users and several functions to evaluate the posterior distribution of all parameters, to estimate the posterior distribution of any contest between items, and to obtain the posterior distribution of the ranks. Three reanalyses of recent studies that used the frequentist Bradley-Terry model are presented. These reanalyses are conducted with the Bayesian models of the bpcs package, and all the code used to fit the models, generate the figures, and the tables are available in the online appendix.

==> sections/6openpractices.tex <==
\section{Open practices statement}

This study was not pre-registered. The data used in the reanalyses can be accessed in the referenced publication or upon request to the authors.

The \texttt{bpcs} package is open-source under the MIT license and the source code can be accessed at the package repository: \url{https://github.com/davidissamattos/bpcs}. Issues or suggestions can be filed in  \url{https://github.com/davidissamattos/bpcs/issues}

The official documentation for the \texttt{bpcs} package can be accessed at:
\url{https://davidissamattos.github.io/bpcs/}.

The reanalyses code can be accessed in the online appendix at:
\url{https://davidissamattos.github.io/bpcs-online-appendix/}
